Hash Adaptive Bloom Filter

Bloom filter is a compact memory-efficient probabilistic data structure supporting membership testing, i.e., to check whether an element is in a given set. However, as Bloom filter maps each element with uniformly random hash functions, few flexibilities are provided even if the information of negative keys (elements are not in the set) are available. The problem gets worse when the misidentification of negative keys brings different costs. To address the above problems, we propose a new Hash Adaptive Bloom Filter (HABF) that supports the customization of hash functions for keys. The key idea of HABF is to customize the hash functions for positive keys (elements are in the set) to avoid negative keys with high cost, and pack customized hash functions into a lightweight data structure named HashExpressor. Then, given an element at query time, HABF follows a two-round pattern to check whether the element is in the set. Further, we theoretically analyze the performance of HABF and bound the expected false positive rate. We conduct extensive experiments on representative datasets, and the results show that HABF outperforms the standard Bloom filter and its cutting-edge variants on the whole in terms of accuracy, construction time, query time, and memory space consumption (Note that source codes are available in [1]).

==> Latex/TechnicalReport.tex <==
\section{appendix}
\label{sec:appendix}
%\subsection{An Example of TPJO algorithm for Optimizing a Collision Key}
%\subsection{Discussion for Bloom filter with different implementations}
%%
%Since the performance of Bloom filter will be affected by different implementations of hash
%function.
%%
%We implement three versions of Bloom filter: BF by using $k$ different kinds of hash functions.
%%
%BF (City64) by using CityHash (64bit version) and BF (XXH128) by using xxHash (128bit version).
%%
%For the latter two implementations, we use different seeds to generate $k$ hash values for accuracy. 
%
%As shown in Fig.~\ref{fig:BFcompare}, the dataset is set to YCSB, under uniform distribution, since the cost of each key is the same, the three versions of Bloom filter ({\it i.e.} BF, BF (City64) and BF (XXH128)) are nearly consistent.
%%
%Under skew distribution, we set the cost distribution of keys to skewness $1.0$, all Bloom filter implementations have fluctuated.
%%
%It demonstrates that even with advanced hash functions like City64 and XXH128, it still can't effectively reduce weighted FPR and are not sensitive to the skew cost distribution.
%%
%\begin{figure}[H]
%\vspace{-2mm}
%\centering
%%\subfigure[On uniform distribution (Shalla)]{
%%\begin{minipage}[t]{0.49\linewidth}
%%\centering
%%\label{fig:BFcompare(a)}
%%\includegraphics[width=1\linewidth]{figure/BFcompare}
%%%\caption{fig1}
%%\vspace{-2mm}
%%\end{minipage}%
%%}%
%%\subfigure[On skew distribution (Shalla)]{
%%\begin{minipage}[t]{0.49\linewidth}
%%\centering
%%\label{fig:BFcompare(b)}
%%\includegraphics[width=1\linewidth]{figure/BFcompare3}
%%%\caption{fig2}
%%\vspace{-2mm}
%%\end{minipage}%
%%}%
%%\\
%\subfigure[On uniform distribution (YCSB)]{
%\begin{minipage}[t]{0.49\linewidth}
%\centering
%\label{fig:BFcompare(a)}
%\includegraphics[width=1\linewidth]{figure/BFcompare2}
%%\caption{fig1}
%\vspace{-2mm}
%\end{minipage}%
%}%
%\subfigure[On skew distribution (YCSB)]{
%\begin{minipage}[t]{0.49\linewidth}
%\centering
%\label{fig:BFcompare(b)}
%\includegraphics[width=1\linewidth]{figure/BFcompare4}
%%\caption{fig2}
%\vspace{-2mm}
%\end{minipage}%
%}%
%\centering
%\vspace{-2mm}
%\caption{Bloom filter with different implementations}
%\label{fig:BFcompare}
%\vspace{-8mm}
%\end{figure}

\subsection{The improved details of HABF}
We have improved the performance of HABF as follows: 1) we have adopted the current strong hash functions (CityHash64, MurmurHash, XXH128) to configure the global hash function set; 2) to improve the space utilization of HashExpressor, we have given the priority to choose the customization hash function set which share the most cells in HashExpressor. 
%
We set the dataset to YCSB with the cost distribution to be uniform and skewness 1.0, respectively. 
%
The compare result are shown in Fig.~\ref{fig:ImproveCompare}.

\begin{figure}[H]
\vspace{-2mm}
\centering
\subfigure[On uniform distribution (YCSB)]{
\begin{minipage}[t]{0.49\linewidth}
\centering
\label{fig:ImproveCompare(a)}
\includegraphics[width=1\linewidth]{figure/ImproveCompared}
%\caption{fig1}
\vspace{-2mm}
\end{minipage}%
}%
\subfigure[On skew distribution (YCSB)]{
\begin{minipage}[t]{0.49\linewidth}
\centering
\label{fig:ImproveCompare(b)}
\includegraphics[width=1\linewidth]{figure/ImproveCompared2}
%\caption{fig2}
\vspace{-2mm}
\end{minipage}%
}%
\centering
\vspace{-2mm}
\caption{Comparison before and after improvement}
\label{fig:ImproveCompare}
\vspace{-8mm}
\end{figure}

\subsection{Proof on Lemma 4.1 and Lemma 4.2}
\textbf{Lemma \ref{lemma:1}} $\forall u \in V, p \in H_0, 0\leq p(u) \leq 1$, have the following relation:
\begin{align}
\label{equa:appendixl1-1}
\prod \limits_{p\in H_0}(1-p(u)) \geq 1- \sum \limits_{p\in H_0}p(u). \tag{\ref{equal:lemma:1}}
\end{align}

\begin{proof}
Let $p_i$ be the distribution of the hash function $h_i$, then Equation (\ref{equa:appendixl1-1}) can be expressed as:
\begin{align}
\label{equa:appendixl1-2}
\prod \limits_{i = 0}^{k}(1-p_i(u)) \geq 1- \sum \limits_{i = 0}^{k}p_i(u). 
\end{align}

%
We denote Equation (\ref{equa:appendixl1-2}) as $\Psi$.
%
Next we use mathematical induction to prove $\Psi$, obviously it holds when $k=0$, we assume that $\Psi$ holds when $k=\alpha-1$, then we have $\prod \limits_{i = 0}^{\alpha-1}(1-p_i(u)) \geq 1- \sum \limits_{i = 0}^{\alpha-1}p_i(u)$ and we can get:

\begin{align}
\label{equa:appendixl1-3}
\prod \limits_{i = 0}^{\alpha}(1-p_i(u)) & = (1-p_\alpha(u))\prod \limits_{i = 0}^{\alpha-1}(1-p_i(u))\notag\\
&=\prod \limits_{i = 0}^{\alpha-1}(1-p_i(u)) - p_\alpha(u) \prod \limits_{i = 0}^{\alpha-1}(1-p_i(u))\notag\\
& \geq 1- \sum \limits_{i = 0}^{\alpha-1}p_i(u) - p_\alpha(u) \prod \limits_{i = 0}^{\alpha-1}(1-p_i(u))\notag\\
& \geq 1- \sum \limits_{i = 0}^{\alpha}p_i(u).
\end{align}
Therefore, $\Psi$ holds when $k=\alpha$, this completes the proof.
\end{proof}

\textbf{Lemma \ref{lemma:2}} $\forall 0\leq x\leq 1$, Function $f(x) = \frac{|S|\cdot x}{\frac{1}{(1-x)^{|S|}}-1}$
is a convex function.
\begin{proof}
We rewrite the $f(x)$ as follows:
\begin{align}
\label{equa:appendixl2-1}
 f(x) = & \frac{|S|\cdot x(1-x)^{|S|}}{1-(1-x)^{|S|}} = \frac{|S|\cdot (1-x)^{|S|}}{\sum \limits_{i = 0}^{|S|-1} (1-x)^i}
\end{align}

Let $\mu = 1-x$ and $\theta = |S|$, so $f(\mu) = \frac{\theta \mu^{\theta}}{\sum \limits_{i = 0}^{\theta-1} \mu^i}$, and we can derive $f'(\mu)$ as follows:

\begin{align}
\label{equa:appendixl2-2}
 f'(\mu) = & \theta\frac{\sum \limits_{i = \theta-1}^{2\theta-2}(2\theta-1-i)\mu^i}{(\sum \limits_{i = 0}^{\theta-1} \mu^i)^2} > 0
\end{align}

Since $f'(x) = \frac{\delta f(\mu)}{\delta \mu} \frac{\delta \mu}{\delta x} = -f'(\mu) < 0$, then we can derive $f''(\mu)$ as follows:
\begin{align}
\label{equa:appendixl2-3}
 f''(\mu)&  = \frac{\theta}{(\sum \limits_{i = 0}^{\theta-1} \mu^i)^4}((\sum \limits_{i = 0}^{\theta-1} \mu^i)^2 \sum \limits_{i = \theta-1}^{2\theta-2}i(2\theta-1-i)\mu^{i-1} \notag\\
  &-2\sum \limits_{i = 0}^{\theta-1} \mu^i\sum \limits_{i = 1}^{\theta-1}i \mu^{i-1}\sum \limits_{i = \theta-1}^{2\theta-2}(2\theta-1-i)\mu^i)\notag\\
  & = \frac{\theta}{(\sum \limits_{i = 0}^{\theta-1} \mu^i)^3}(\sum \limits_{i = 0}^{\theta-1} \mu^i \sum \limits_{i = \theta-1}^{2\theta-2}i(2\theta-1-i)\mu^{i-1} \notag\\
  &-2\sum \limits_{i = 0}^{\theta-1}i \mu^i\sum \limits_{i = \theta-1}^{2\theta-2}(2\theta-1-i)\mu^{i-1})
\end{align}

Next, we compare $\sum \limits_{i = 0}^{\theta-1}i \mu^i$ with $\frac{\theta-1}{2} \sum \limits_{i = 0}^{\theta-1}\mu^i$,

\begin{align}
\label{equa:appendixl2-4}
 & \frac{\theta-1}{2} \sum \limits_{i = 0}^{\theta-1}\mu^i - \sum \limits_{i = 0}^{\theta-1}i \mu^i \notag\\
 =& \sum \limits_{i = 0}^{\theta-1}(\frac{\theta-1}{2} - i)\mu^i \notag\\
 =& \sum \limits_{i = 0}^{\frac{\theta-1}{2}}(\frac{\theta-1}{2} - i)(\mu^i - \mu^{\theta - 1 - i})
\end{align}

Since $0\leq \mu \leq 1$, we have $\sum \limits_{i = 0}^{\theta-1}i \mu^{i}  < \frac{\theta-1}{2} \sum \limits_{i = 0}^{\theta-1}\mu^{i}$. According to Equation (\ref{equa:appendixl2-3}), we have:

\begin{align}
\label{equa:appendixl2-5}
f''(\mu) & > \frac{\theta}{(\sum \limits_{i = 0}^{\theta-1} \mu^i)^3}(\sum \limits_{i = 0}^{\theta-1} \mu^i \sum \limits_{i = \theta-1}^{2\theta-2}i(2\theta-1-i)\mu^{i-1} \notag\\
  &-(\theta-1) \sum \limits_{i = 0}^{\theta-1}\mu^{i}\sum \limits_{i = \theta-1}^{2\theta-2}(2\theta-1-i)\mu^{i-1})\notag\\
& = \frac{\theta}{(\sum \limits_{i = 0}^{\theta-1} \mu^i)^2}\sum \limits_{i = \theta-1}^{2\theta-2}(i-(\theta-1))(2\theta-1-i)\mu^{i-1}
\end{align}

Therefore, $f''(\mu) > 0$ and $f''(x) = \frac{\delta^2 f(\mu)}{\delta^2 \mu}(\frac{\delta \mu}{\delta x})^2 + \frac{\delta f(\mu)}{\delta \mu}(\frac{\delta^2 \mu}{\delta^2 x})= f''(\mu) > 0$. Since $f'(x)<0,f''(x)>0$, $f(x)$ is a convex function.

\end{proof}

\subsection{Analysis of $P'_c$}
%Next, we analyze $P'_c$.
%
To simplify the analysis, we assume that each bit in Bloom filter is set to $0$ with probability $p_0$ and $1$ with probability $ 1 - p_0$.
%
Note that we do not consider the case of $cost$ $exchange$.
%
When all buckets mapped by $e_{sk}$ through all hash functions in $H_c$ are \emph{conflict after adjustment}, we cannot adjust the hash functions of $e_{sk}$, so we get
%
\begin{align}
P'_c = 1 - \prod \limits_{h \in H_c(e_{sk})}(1-(1-p_0^{k-1})^{\chi(h(e_{sk}))}),
\end{align}
%
where $\chi(i)$ represents the number of keys in the $i^{th}$ bucket of $\Gamma$.
Moreover, according to average value inequality, we have
\begin{align}
1-P'_c \leq & (\frac{|H|-k - \sum \limits_{h \in H_c}(1-p_0^{k-1})^{\chi(h(e_{sk}))}}{|H|-k})^{|H|-k} \notag\\
 \leq & (1-\frac{1}{|H|-k}\sum \limits_{h \in H_c}(1-p_0^{k-1})^{\chi(h(e_{sk}))})^{|H|-k} \notag\\
\leq & (1-\prod \limits_{h \in H_c}(1-p_0^{k-1})^{\frac{\chi(h(e_{sk}))}{|H|-k}})^{|H|-k}.
\end{align}
%
It is easy to prove that: $ \forall 0<\alpha<1, \beta \in \mathbb{N}, (1-\alpha)^\beta < 1-\alpha ^\beta$, which is similar to Lemma \ref{lemma:1}, then we have
%
\begin{align}
1-P'_c < &  1-(1-p_0^{k-1})^{\sum \limits_{h \in H_c}\chi(h(e_{sk}))} \notag\\
P'_c > & (1-p_0^{k-1})^{\sum \limits_{h \in H_c}\chi(h(e_{sk}))}.
\end{align}
%
Since function $g''(x) = (1-p_0^{k-1})^{x}$ is a convex function, by the Jensen inequality, we get
%
\begin{align}
E(P'_c) > (1-p_0^{k-1})^{E(\sum \limits_{h \in H_c}\chi(h(e_{sk})))}.
\end{align}

Let $\psi = \sum \limits_{h \in H_c}\chi(h(e_{sk}))$, and we assume that $\forall h \in H, e_{sk} \in S$, for a certain unit $u$ in $V$, the probability that $u$ is mapped by $e_{sk}$ through $h$ is only determined by $p(u)$, so we have
%
\begin{align}
E(\psi) =& E(\sum \limits_{u = 1}^{m} \sum \limits_{p \in H_c}\chi(u)p(u)) = E(\sum \limits_{u = 1}^{m}\chi(u) \sum \limits_{p \in H_c}p(u)),
\end{align}
where $\chi(u) = |O|\sum \limits_{p' \in H_0}p'(u)$, for $\forall p_\alpha \in H_0$, $p_\gamma \in H_c$, $p_\alpha$ and $p_\gamma$ are independent of each other, we have
%
\begin{align}
E(\psi) =& \sum \limits_{u = 1}^{m}|O| E(\sum \limits_{p \in H_0}p(u)) \cdot E(\sum \limits_{p \in H_c}p(u)) \notag\\
<& \sum \limits_{u = 1}^{m} \frac{|O|}{4}(\sum \limits_{p \in H}E(p(u)))^2 = \frac{|O|\cdot |H|^2}{4m}.
\end{align}
%
Since $0 < (1-p_0^{k-1}) < 1$, then
\begin{align}
E(P'_c) > (1-p_0^{k-1})^{\frac{|O|\cdot |H|^2}{4m}}.
\end{align}
\red{
\subsection{Analysis of HABF Under Insertion Workloads}
%
In this subsection, we theoretically analyze the performance of HABF under insertion workloads.
%
Let the cost of the $i^{th}$ bit of Bloom filter be $\Theta'(i)$. %due to the limit of space size, we can only customize a small part of hash functions for massive inserted keys, we only consider the scenario that $\Theta'$ is skew.
%
If $\alpha$ keys have inserted, the probability that a certain bit remains '0' is $(1-\frac{1}{m})^{k\alpha}$.}

\red{
%%
Thus, for Bloom filter, the overall cost of false positives in $O$ can be derived as
\begin{align}
C_{bf} = \sum \limits_{i = 1}^m (1-(1-\frac{1}{m})^{k\alpha})\Theta'(i).
\end{align}}

\red{
%%
For HABF, In this scenario, when a bit $x$ is inserted, we compares its cost with the preset threshold $\tau$.
%
If $\Theta'(x) \geq \tau$, we try to customize the hash functions of inserted positive keys to prevent setting $x$ to '1'.
%
We denote the probability that a bit $i$ is prevented from be setting to '1' as $P(i)$, then for HABF, the overall cost of false positives in $O$ can be derived as
\begin{align}
\label{equa:dynamic3}
C_{habf} = \sum \limits_{i = 1}^m (1-(1-\frac{1}{m}+\frac{P(i)}{m})^{k\alpha})\Theta'(i).
\end{align}}

\red{
%%
As per Equation (\ref{equa:dynamic3}), it is obvious that $C_{habf} \leq C_{bf}$.
%
Since $(1-\frac{1-P(i)}{m}) < 1, \lim\limits_{\alpha\to+\infty}C_{habf} = \sum\limits_{i = 1}^m \Theta'(i)$, which means $C_{habf}$ will also tend to reach the max overall cost but at a lower speed.
%
Next we analyze $P$ in detail. We denote $P_c$ as the probability that a inserted key can customize its hash functions successfully and $P_c$ as the probability that the customization results can be inserted into HashExpressor, $P_c$ and $P_s$ are independent of each other, then we have
\begin{align}
\label{equa:dynamic4}
P(i) = Pr(\Theta'(i) > \tau)\cdot P_c\cdot P_s.
\end{align}
%
We set $\tau$ to the $h^{th}$ highest value in $\Theta'(i)$ for $i=1, 2, ..., m$, then $Pr(\Theta'(i) > \tau) = \frac{h}{m}$.
%
Considering $P_c$, for a inserted key $e$, as there are $|H_c|$ hash functions for selection, if there exists a hash function which can be used to mapped to a bit with cost below $\tau$, the customization is undoubtedly successful, then
%%
%In practical, only a small part of hash functions for massive inserted keys are customized, we assume the underly distribution of '1' is ideal uniform, then
\begin{align}
\label{equa:dynamic5}
P_c = 1-(\frac{h}{m})^{|H_c|}.
\end{align}
Considering $P_s$ related to the number of customized keys, which we denote as $t$, according to Equation (\ref{equa:8}) and Lemma \ref{lemma:1}, we have
\begin{align}
\label{equa:dynamic6}
P_s  > (1-\frac{kt+k}{\omega})^k > 1-\frac{k^2(t+1)}{\omega}.
\end{align}
As per Equation (\ref{equa:dynamic4}), we have $E(t) = k\alpha\cdot \frac{h}{m}\cdot P_c \cdot E(P_s)$, then we have can derive
\begin{align}
\label{equa:dynamic7}
E(P_s) > & 1-\frac{k^2(E(t)+1)}{\omega}\notag\\
>& 1-\frac{k^2( \frac{k\alpha hP_c}{m} \cdot E(P_s)+1)}{\omega}\notag\\
>& \frac{(\omega+k^2)m}{\omega m+k^3\alpha hP_c}.
\end{align}
As per Equation (\ref{equa:dynamic4}) and (\ref{equa:dynamic7}), Then we have
\begin{align}
\label{equa:dynamic8}
E(P(i)) > \frac{(\omega+k^2)}{\frac{\omega m}{P_c h}+k^3\alpha}.
\end{align}} 

==> Latex/background.tex <==
\section{Background}
\begin{table}[t]
\small
  \caption{Notations}
  \begin{center}
    \begin{tabularx}{8cm}{|r|p{6.3cm}|}
      \hline
      \textbf{Symbol} & \textbf{Description} \\
      \hline
      $T$ & {Time span of observation} \\
      \hline
      $L$ & {Length of a timeslot} \\
      \hline
      $\tau(x,y)$ & { Time span between data points $x$ and $y$.} \\
      \hline
      $T_{th}$ & {Threshold of persistence} \\
      \hline
      $l$ & {Length of ID in bits} \\
      \hline
      $p$ & {Length of fingerprint in bytes} \\
      \hline
      $N$ & {Number of all items in } \\
      \hline
      $U$ & {Universal set of all distinct items}\\
      \hline
      $n_i$ & {Number of distinct items in $S_i$}\\
      \hline
      $N_i$ & {Number of items in $S_i$} \\
      \hline
      $n$ & {Number of distinct items} \\
      \hline
      $f_i(x)$  & {Frequency of element $x$ in $S_i$}\\
      \hline
      $f(x)$  & {Frequency of element $x$ in $\bigcup_{i \in [m]}S_i$}\\
      \hline
      $h_f(\cdot)$  & {Hash function of fingerprint}\\
      \hline
    \end{tabularx}
 \end{center}
 \label{Tab:Notation}
% \vspace{-2em}
\end{table}

\textbf{Ternary search tree(TST): }
%
Ternary search tree(TST)\cite{uth1973art} is a variant of trie tree data structure.
%
Different from a standard trie tree, each node of ternary search tree have only three child nodes and extremely space efficient.
%
Of the three child nodes of each node, the first one points to a node whose value is less than the current node's value, the second one node points to the node with value equal to the current node's value and the third node points to the node whose value is greater than the current node's value.
%
%
By using ternary search tree, the search complexities can be brought to nearly optimal (key length).
%

\textbf{Insertion procedure:} Suppose each item has an $l$-byte ID $I = \{i_1,i_2,\cdots,i_l\}$.
%
To insert an item into TST, we need to compare the bytes of the ID with the value of nodes in TST.
%
Let $i_c$ denote the current byte in the ID to be compared, which is initialized to the first byte.
%
Let the $\nu$ denote a node in TST, which is initially set to the root node of TST. 
%

We first compare $i_c$ with $\nu$ and perform actions according to the result of the comparison.
%
Note that if the node $\nu$ does not exist, we new a node of the same value as the compared byte of the ID and continue the comparison process.
%
If $i_c$ is equals to $\nu$, we set $i_c$ to the next byte by setting $c=c+1$ and $\nu$ to its middle child and then repeat the comparing process until all bytes of the ID have been .
%

If $i_c$ is less than $\nu$, we set $\nu$ to be the left child of the $\nu$ and then repeat the comparing process.
%
If $i_c$ is larger than $\nu$, we set $\nu$ to be the right child of the $\nu$ and then repeat the comparing process and repeat the comparing process.
%
To insert the ID into the ID filter, we follow the steps of insert items into TST except we allow a of no other item of the same.

\begin{algorithm} 
\caption{Insertion Procedure of TST (INSERT-TST)} \label{alg:INSERT-TST}
\begin{algorithmic}[1]
\Require ID$: [i_1,i_2,\cdots,i_l]$, $c = 1$, TST, $\nu$ = TST.root;\;
\Procedure{INSERT-TST}{$c,TST,\nu$}
\While{ $c \leq l$} %
	\If{ $\nu ==  NUll$ }
		\State create a new node with value $i_c$ 
		\State set $c = c + 1$ 
	\Else
		\If {$i_c == \nu.value$}
			\State $c = c+1,\nu=\nu.middle$\;
		\ElsIf{$i_c < \nu.value$}
				\State $\nu=\nu.left$\;
		\Else 
				\State $\nu = \nu.right$
		\EndIf
	\EndIf
\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

%
%\begin{algorithm}[h]
%%\small
%\caption{Insertion Procedure of TST}
%\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
%%\KwIn{ ID Filter TST and ID $I = \{ i_1,i_2,\cdots,i_l \}$}
%%\KwOut{Semi-matching $M$ on $G$ with minimum number of entries.}
%%\Indm\nonl\printlcs{$b,X,i,j$}\\
%%\Indp
%\begin{algorithmic}
%$i_c = i_1$, $\nu$ = TST.root;\;
%%\Function{Distance}{$x, y$}
% \While{ $c \leq l$} %
%{
%	\If{ $\nu ==  NUll$ }
%	{
%		create a new node with value $i_c$ \;
%		set $c = c + 1$ \;
%	}
%	\Else
%	{
%		\If {$i_c == \nu.value$}
%		{
%			$c = c+1,\nu=\nu.middle$\;
%		}
%		\Else
%		{
%			\If{$i_c <= \nu.value$}
%			{
%				$\nu=\nu.left$\;
%			}	
%			\Else
%			{
%				$\nu = \nu.right$ \;
%			}
%		}
%	}
%}
%%
%\end{algorithmic}
%\label{alg:insertTST}
%\end{algorithm}


\textbf{Local Sensitive Hashing (LSH):}
\red{
Locality-Sensitive Hashing (LSH)\cite{gionis1999similarity} is an algorithm for solving the approximate or exact Near Neighbor Search in high dimensional spaces. 
%
A locality-preserving hashing is a hash function f that maps a point or points in a multidimensional coordinate space to a scalar value, such that if we have three points A, B and C such that $|A-B|<|B-C| \Rightarrow |f(A)-f(B)|<|f(B)-|f(C)|$.
%
In other words, these are hash functions where the relative distance between the input values is preserved in the relative distance between of the output hash values; input values that are closer to each other will produce output hash values that are closer to each other.}
%
\begin{figure}
  \centering
  \includegraphics[width=0.4\textwidth]{fig/Ternary-Search-Tree.png}
  \caption{Example of Ternary Search Tree(TST)}
\end{figure}


